Efficient Estimation for Staggered Rollout Designs

We study estimation of causal effects in staggered rollout designs, i.e. settings where there is staggered treatment adoption and the timing of treatment is as-good-as randomly assigned. We derive the most efficient estimator in a class of estimators that nests several popular generalized difference-in-differences methods. A feasible plug-in version of the efficient estimator is asymptotically unbiased with efficiency (weakly) dominating that of existing approaches. We provide both $t$-based and permutation-test-based methods for inference. In an application to a training program for police officers, confidence intervals for the proposed estimator are as much as eight times shorter than for existing approaches.

==> Tables/Wood-et-al-sims/2-period-sims-sd-ratios.tex <==
\captionsetup[table]{labelformat=empty,skip=1pt}
\begin{longtable}{rrrrrrrr}
\toprule
& & & & & \multicolumn{3}{c}{SD Relative to Plug-In} \\ 
 \cmidrule(lr){6-8}
N\_1 & N\_0 & rho & gamma & betastar & PlugIn & DiD & DiM \\ 
\midrule
1000 & 1000 & 0.99 & 0.0 & $0.99$ & $1.00$ & $1.00$ & $7.09$ \\ 
1000 & 1000 & 0.99 & 0.5 & $1.24$ & $1.00$ & $1.71$ & $7.07$ \\ 
1000 & 1000 & 0.50 & 0.0 & $0.52$ & $1.00$ & $1.13$ & $1.15$ \\ 
1000 & 1000 & 0.50 & 0.5 & $0.65$ & $1.00$ & $1.04$ & $1.15$ \\ 
1000 & 1000 & 0.00 & 0.0 & $-0.03$ & $1.00$ & $1.45$ & $1.00$ \\ 
1000 & 1000 & 0.00 & 0.5 & $-0.03$ & $1.00$ & $1.31$ & $1.00$ \\ 
25 & 25 & 0.99 & 0.0 & $0.97$ & $1.00$ & $0.99$ & $6.58$ \\ 
25 & 25 & 0.99 & 0.5 & $1.22$ & $1.00$ & $1.47$ & $6.31$ \\ 
25 & 25 & 0.50 & 0.0 & $0.41$ & $1.00$ & $1.21$ & $1.10$ \\ 
25 & 25 & 0.50 & 0.5 & $0.51$ & $1.00$ & $1.08$ & $1.10$ \\ 
25 & 25 & 0.00 & 0.0 & $0.10$ & $1.00$ & $1.35$ & $0.98$ \\ 
25 & 25 & 0.00 & 0.5 & $0.13$ & $1.00$ & $1.22$ & $0.98$ \\ 
\bottomrule
\end{longtable}



==> Tables/Wood-et-al-sims/2-period-sims.tex <==
\captionsetup[table]{labelformat=empty,skip=1pt}
\begin{longtable}{rrrrrrrrrrrrrrrr}
\toprule
& & & & \multicolumn{3}{c}{Bias} & \multicolumn{3}{c}{SD} & \multicolumn{3}{c}{Coverage} & \multicolumn{3}{c}{FRT Size} \\ 
 \cmidrule(lr){5-7}\cmidrule(lr){8-10}\cmidrule(lr){11-13}\cmidrule(lr){14-16}
N\_1 & N\_0 & rho & gamma & PlugIn & DiD & DiM & PlugIn & DiD & DiM & PlugIn & DiD & DiM & PlugIn & DiD & DiM \\ 
\midrule
1000 & 1000 & 0.99 & 0.0 & $0.00$ & $0.00$ & $-0.00$ & $0.01$ & $0.01$ & $0.04$ & $0.95$ & $0.95$ & $0.95$ & $0.05$ & $0.05$ & $0.05$ \\ 
1000 & 1000 & 0.99 & 0.5 & $0.00$ & $0.00$ & $-0.00$ & $0.01$ & $0.01$ & $0.06$ & $0.95$ & $0.95$ & $0.95$ & $0.04$ & $0.06$ & $0.05$ \\ 
1000 & 1000 & 0.50 & 0.0 & $0.00$ & $0.00$ & $0.00$ & $0.04$ & $0.04$ & $0.05$ & $0.94$ & $0.95$ & $0.94$ & $0.06$ & $0.05$ & $0.05$ \\ 
1000 & 1000 & 0.50 & 0.5 & $0.00$ & $0.00$ & $0.00$ & $0.05$ & $0.05$ & $0.06$ & $0.95$ & $0.95$ & $0.95$ & $0.06$ & $0.05$ & $0.05$ \\ 
1000 & 1000 & 0.00 & 0.0 & $-0.00$ & $0.00$ & $-0.00$ & $0.04$ & $0.07$ & $0.04$ & $0.95$ & $0.94$ & $0.95$ & $0.05$ & $0.06$ & $0.05$ \\ 
1000 & 1000 & 0.00 & 0.5 & $-0.00$ & $0.00$ & $-0.00$ & $0.06$ & $0.07$ & $0.06$ & $0.95$ & $0.95$ & $0.95$ & $0.04$ & $0.05$ & $0.05$ \\ 
25 & 25 & 0.99 & 0.0 & $0.00$ & $0.00$ & $-0.03$ & $0.04$ & $0.04$ & $0.27$ & $0.94$ & $0.94$ & $0.94$ & $0.04$ & $0.05$ & $0.06$ \\ 
25 & 25 & 0.99 & 0.5 & $0.00$ & $-0.01$ & $-0.04$ & $0.05$ & $0.08$ & $0.34$ & $0.92$ & $0.93$ & $0.93$ & $0.06$ & $0.06$ & $0.06$ \\ 
25 & 25 & 0.50 & 0.0 & $-0.01$ & $0.02$ & $-0.02$ & $0.24$ & $0.29$ & $0.26$ & $0.94$ & $0.95$ & $0.94$ & $0.04$ & $0.04$ & $0.05$ \\ 
25 & 25 & 0.50 & 0.5 & $-0.01$ & $0.01$ & $-0.03$ & $0.30$ & $0.32$ & $0.33$ & $0.94$ & $0.95$ & $0.94$ & $0.04$ & $0.04$ & $0.05$ \\ 
25 & 25 & 0.00 & 0.0 & $-0.03$ & $-0.02$ & $-0.03$ & $0.28$ & $0.38$ & $0.27$ & $0.93$ & $0.95$ & $0.93$ & $0.06$ & $0.04$ & $0.06$ \\ 
25 & 25 & 0.00 & 0.5 & $-0.04$ & $-0.02$ & $-0.04$ & $0.35$ & $0.42$ & $0.34$ & $0.93$ & $0.94$ & $0.94$ & $0.06$ & $0.05$ & $0.06$ \\ 
\bottomrule
\end{longtable}



==> Tables/Wood-et-al-sims/coverage-table-complaints-with-lags.tex <==
\begin{longtable}{llrrrr}
\toprule
Estimator & Estimand & Bias & Coverage & Mean SE & SD \\ 
\midrule
PlugIn & calendar & 0.01 & 0.94 & 0.26 & 0.27 \\ 
PlugIn & cohort & 0.01 & 0.92 & 0.26 & 0.27 \\ 
PlugIn & ES0 & 0.01 & 0.95 & 0.32 & 0.33 \\ 
PlugIn & cohort & 0.01 & 0.93 & 0.24 & 0.25 \\ 
PlugIn with 10 lags & calendar & 0.00 & 0.93 & 0.24 & 0.26 \\ 
PlugIn with 10 lags & cohort & 0.02 & 0.91 & 0.25 & 0.26 \\ 
PlugIn with 10 lags & ES0 & 0.03 & 0.95 & 0.32 & 0.32 \\ 
PlugIn with 10 lags & cohort & 0.01 & 0.93 & 0.23 & 0.24 \\ 
\bottomrule
\caption{Simulation Results Using Baseline $\hat{X}$ and Variant with 10 Lags}
\end{longtable}



==> Tables/Wood-et-al-sims/coverage-table-full-data.tex <==
\captionsetup[table]{labelformat=empty,skip=1pt}
\begin{longtable}{llrrrrl}
\toprule
Estimator & Estimand & Bias & Coverage & Mean SE & SD & Estimat \\ 
\midrule
Efficient & calendar & 0.00 & 0.93 & 0.27 & 0.29 & PlugIn \\ 
Efficient & cohort & 0.00 & 0.92 & 0.24 & 0.24 & PlugIn \\ 
Efficient & ES0 & 0.01 & 0.94 & 0.26 & 0.27 & PlugIn \\ 
Efficient & simple & 0.00 & 0.92 & 0.22 & 0.22 & PlugIn \\ 
CS & calendar & 0.01 & 0.76 & 0.54 & 0.85 & CS \\ 
CS/CdH & ES0 & 0.01 & 0.94 & 0.36 & 0.36 & CS \\ 
CS & cohort & -0.01 & 0.95 & 0.41 & 0.41 & CS \\ 
CS & simple & -0.01 & 0.96 & 0.41 & 0.40 & CS \\ 
\bottomrule
\end{longtable}



==> Tables/Wood-et-al-sims/coverage-table-long-A0-complaints-het-effects.tex <==
\captionsetup[table]{labelformat=empty,skip=1pt}
\begin{longtable}{llrrrrr}
\toprule
Estimator & Estimand & Bias & Coverage & FRT Size & Mean SE & SD \\ 
\midrule
PlugIn - Long X & calendar & -3.30 & 0.07 & 0.02 & 0.34 & 137.65 \\ 
PlugIn - Long X & cohort & 1.83 & 0.06 & 0.01 & 0.26 & 95.20 \\ 
PlugIn - Long X & ES0 & -20.56 & 0.05 & 0.02 & 0.36 & 403.98 \\ 
PlugIn - Long X & simple & -0.16 & 0.06 & 0.01 & 0.28 & 100.03 \\ 
PlugIn & calendar & 0.00 & 0.98 & 0.02 & 0.45 & 0.38 \\ 
PlugIn & cohort & 0.00 & 0.99 & 0.01 & 0.39 & 0.28 \\ 
PlugIn & ES0 & 0.00 & 0.99 & 0.01 & 0.42 & 0.31 \\ 
PlugIn & simple & 0.00 & 1.00 & 0.00 & 0.38 & 0.26 \\ 
 \bottomrule
\end{longtable}



==> Tables/Wood-et-al-sims/coverage-table-long-A0-force-annual-t-and-g.tex <==
\captionsetup[table]{labelformat=empty,skip=1pt}
\begin{longtable}{llrrrrr}
\toprule
Estimator & Estimand & Bias & Coverage & FRT Size & Mean SE & SD \\ 
\midrule
PlugIn - Long X & calendar & 0.29 & 0.93 & 0.06 & 2.57 & 2.66 \\ 
PlugIn - Long X & cohort & 0.30 & 0.93 & 0.06 & 3.05 & 3.20 \\ 
PlugIn - Long X & ES0 & 0.34 & 0.93 & 0.06 & 2.43 & 2.55 \\ 
PlugIn - Long X & simple & 0.32 & 0.93 & 0.06 & 2.97 & 3.11 \\ 
PlugIn & calendar & -0.16 & 0.95 & 0.05 & 2.71 & 2.69 \\ 
PlugIn & cohort & -0.17 & 0.94 & 0.05 & 3.23 & 3.24 \\ 
PlugIn & ES0 & -0.06 & 0.94 & 0.06 & 2.54 & 2.57 \\ 
PlugIn & simple & -0.18 & 0.94 & 0.05 & 3.15 & 3.16 \\ 
 \bottomrule
\end{longtable}



==> Tables/Wood-et-al-sims/coverage-table-long-A0-force.tex <==
\captionsetup[table]{labelformat=empty,skip=1pt}
\begin{longtable}{llrrrrr}
\toprule
Estimator & Estimand & Bias & Coverage & FRT Size & Mean SE & SD \\ 
\midrule
PlugIn - Long X & calendar & 2.96 & 0.01 & 0.05 & 0.11 & 25.76 \\ 
PlugIn - Long X & cohort & 0.96 & 0.01 & 0.06 & 0.06 & 36.55 \\ 
PlugIn - Long X & ES0 & 0.87 & 0.03 & 0.06 & 0.27 & 65.96 \\ 
PlugIn - Long X & simple & 2.29 & 0.00 & 0.05 & 0.06 & 21.86 \\ 
PlugIn & calendar & 0.02 & 0.95 & 0.05 & 0.31 & 0.32 \\ 
PlugIn & cohort & 0.02 & 0.92 & 0.05 & 0.33 & 0.34 \\ 
PlugIn & ES0 & -0.02 & 0.95 & 0.05 & 0.34 & 0.34 \\ 
PlugIn & simple & 0.01 & 0.92 & 0.05 & 0.30 & 0.31 \\ 
 \bottomrule
\end{longtable}



==> Tables/Wood-et-al-sims/coverage-table-long-A0-sustained-annual-t-and-g.tex <==
\captionsetup[table]{labelformat=empty,skip=1pt}
\begin{longtable}{llrrrrr}
\toprule
Estimator & Estimand & Bias & Coverage & FRT Size & Mean SE & SD \\ 
\midrule
PlugIn - Long X & calendar & 0.21 & 0.88 & 0.06 & 0.50 & 0.54 \\ 
PlugIn - Long X & cohort & 0.22 & 0.88 & 0.06 & 0.58 & 0.64 \\ 
PlugIn - Long X & ES0 & 0.30 & 0.88 & 0.06 & 0.64 & 0.70 \\ 
PlugIn - Long X & simple & 0.23 & 0.87 & 0.06 & 0.56 & 0.62 \\ 
PlugIn & calendar & 0.02 & 0.94 & 0.05 & 0.52 & 0.53 \\ 
PlugIn & cohort & 0.02 & 0.94 & 0.05 & 0.60 & 0.63 \\ 
PlugIn & ES0 & 0.04 & 0.94 & 0.06 & 0.67 & 0.67 \\ 
PlugIn & simple & 0.02 & 0.94 & 0.05 & 0.59 & 0.61 \\ 
 \bottomrule
\end{longtable}



==> Tables/Wood-et-al-sims/coverage-table-long-A0-sustained.tex <==
\captionsetup[table]{labelformat=empty,skip=1pt}
\begin{longtable}{llrrrrr}
\toprule
Estimator & Estimand & Bias & Coverage & FRT Size & Mean SE & SD \\ 
\midrule
PlugIn - Long X & calendar & 0.26 & 0.00 & 0.05 & 0.03 & 0.05 \\ 
PlugIn - Long X & cohort & 0.21 & 0.00 & 0.05 & 0.01 & 0.01 \\ 
PlugIn - Long X & ES0 & 0.38 & 0.00 & 0.05 & 0.08 & 0.10 \\ 
PlugIn - Long X & simple & 0.23 & 0.00 & 0.05 & 0.01 & 0.01 \\ 
PlugIn & calendar & 0.00 & 0.95 & 0.06 & 0.05 & 0.06 \\ 
PlugIn & cohort & 0.00 & 0.94 & 0.04 & 0.04 & 0.04 \\ 
PlugIn & ES0 & 0.00 & 0.94 & 0.06 & 0.10 & 0.10 \\ 
PlugIn & simple & 0.00 & 0.94 & 0.04 & 0.04 & 0.04 \\ 
 \bottomrule
\end{longtable}



==> Tables/Wood-et-al-sims/sd-ratio-table-complaints-het-effects.tex <==
\captionsetup[table]{labelformat=empty,skip=1pt}
\begin{longtable}{lrr}
\toprule
 & \multicolumn{2}{c}{Ratio of SD to Plug-In} \\ 
 \cmidrule(lr){2-3}
Estimand & CS & SA \\ 
\midrule
calendar & $1.53$ & $4.01$ \\ 
cohort & $1.67$ & $5.72$ \\ 
ES0 & $1.38$ & $3.01$ \\ 
simple & $1.80$ & $6.62$ \\ 
 \bottomrule
\end{longtable}



==> Tables/Wood-et-al-sims/sd-ratio-table-complaints-with-lags.tex <==
\begin{longtable}{lr}
\toprule
Estimands & Ratio of SDs \\ 
\midrule
calendar & $0.97$ \\ 
cohort & $0.99$ \\ 
ES0 & $0.99$ \\ 
simple & $0.98$ \\ 
\bottomrule
\caption{Ratio of SD Using 10 Lags Versus Baseline}
\end{longtable}



==> Tables/Wood-et-al-sims/sd-ratio-table-full-data.tex <==
\captionsetup[table]{labelformat=empty,skip=1pt}
\begin{longtable}{lr}
\toprule
Estimand & Ratio of SDs \\ 
\midrule
calendar & $2.97$ \\ 
cohort & $1.67$ \\ 
ES0 & $1.36$ \\ 
simple & $1.82$ \\ 
\bottomrule
\end{longtable}



==> Tables/wood-et-al-application-percentage-effects.tex <==
\captionsetup[table]{labelformat=empty,skip=1pt}
\begin{longtable}{llrrrrrrrr}
\toprule
& & & \multicolumn{3}{c}{Plug-In} & \multicolumn{3}{c}{CS} & \\ 
 \cmidrule(lr){4-6}\cmidrule(lr){7-9}
Outcome & Estimand & Pre-treatment Mean & Estimate & LB & UB & Estimate & LB & UB & CI Ratio \\ 
\midrule
complaints & simple & $0.049$ & $-2.3\%$ & $-10.7\%$ & $6.1\%$ & $-10.5\%$ & $-26.1\%$ & $5.1\%$ & $1.9$ \\ 
complaints & calendar & $0.049$ & $-3.8\%$ & $-14.0\%$ & $6.4\%$ & $-24.1\%$ & $-56.3\%$ & $8.1\%$ & $3.2$ \\ 
complaints & cohort & $0.049$ & $-2.2\%$ & $-11.2\%$ & $6.8\%$ & $-9.1\%$ & $-24.8\%$ & $6.7\%$ & $1.8$ \\ 
sustained & simple & $0.004$ & $-7.4\%$ & $-23.0\%$ & $8.1\%$ & $26.5\%$ & $-43.6\%$ & $96.6\%$ & $4.5$ \\ 
sustained & calendar & $0.004$ & $-16.7\%$ & $-30.0\%$ & $-3.4\%$ & $-1.2\%$ & $-75.5\%$ & $73.1\%$ & $5.6$ \\ 
sustained & cohort & $0.004$ & $-6.7\%$ & $-22.4\%$ & $9.1\%$ & $29.2\%$ & $-40.7\%$ & $99.2\%$ & $4.4$ \\ 
force & simple & $0.048$ & $-14.5\%$ & $-29.2\%$ & $0.1\%$ & $-22.3\%$ & $-42.9\%$ & $-1.6\%$ & $1.4$ \\ 
force & calendar & $0.048$ & $-12.7\%$ & $-25.5\%$ & $0.1\%$ & $-38.1\%$ & $-71.8\%$ & $-4.3\%$ & $2.6$ \\ 
force & cohort & $0.048$ & $-15.7\%$ & $-31.3\%$ & $-0.2\%$ & $-22.1\%$ & $-42.8\%$ & $-1.4\%$ & $1.3$ \\ 
\bottomrule
\end{longtable}



==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
 
sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -pdf \"$_[0]\"" );
    }
}
